Patchview: LLM-Powered Worldbuilding with Generative Dust and Magnet Visualization

Large language models (LLMs) can help writers build story worlds by generating world elements, such as factions, characters, and locations. However, making sense of many generated elements can be overwhelming. Moreover, if the user wants to precisely control aspects of generated elements that are difficult to specify verbally, prompting alone may be insufficient. We introduce Patchview, a customizable LLM-powered system that visually aids worldbuilding by allowing users to interact with story concepts and elements through the physical metaphor of magnets and dust. Elements in Patchview are visually dragged closer to concepts with high relevance, facilitating sensemaking. The user can also steer the generation with verbally elusive concepts by indicating the desired position of the element between concepts. When the user disagrees with the LLM's visualization and generation, they can correct those by repositioning the element. These corrections can be used to align the LLM's future behaviors to the user's perception. With a user study, we show that Patchview supports the sensemaking of world elements and steering of element generation, facilitating exploration during the worldbuilding process. Patchview provides insights on how customizable visual representation can help sensemake, steer, and align generative AI model behaviors with the user's intentions.

==> sections/00_teaserfigure.tex <==
  \includegraphics[width=\textwidth]{figures/patchview_teaser.pdf}
  \caption{For generating story world elements with LLMs, \sys{} leverages a dust and magnet visual representation to help users a) sensemake, b) steer, and c) correct LLM generation. a) In dust and magnet visual representation, user-defined concepts serve as ``magnets’’ (larger dark circles), attracting ``dust particle’’ elements (smaller light circles) more strongly if an element is more relevant to the concept. Note that we only show partial excerpts of magnets due to the limited space. b) By placing a red marker between magnets, the user can steer the generation with a mix of different concepts. c) When LLM behaviors (steering, recognition) do not align with the user’s perception, the user can correct them simply by moving the element, either 1) revising the element position or 2) re-steering generation to rewrite the element. The corrected placement will be fed into the LLM pipeline as an example to improve future steering and recognition.}
  \Description{The figure demonstrates how LLMs can generate elements for a story world using a "dust and magnet" visual representation. The image is divided into three parts: a) Sensemaking generation of world elements: This section shows how LLM-generated story elements (represented as smaller light circles or "dust particles") are attracted to user-defined concepts (represented as larger dark circles or "magnets"). The relevance of an element to a concept determines how strongly it is attracted. Three character descriptions are provided as examples, with the two views. The first view has two concepts, "Good" and "Evil." The second view has three concepts of factions, "The League of the Blind... use psychic abilities...", "The Order of the Open Hand... embracing all senses...", and "The Sighted Saviors, a militant order... enforcing rationalism..." The first character is placed close to "Good" in the first view, and placed in the middle of three factions, with the description of "Morgan Fairweather, 41, is a thoughtful druid adept in communing with nature, who has mediated disputes between the mystics and rationalists for years. Though formally aligned with the Open Hand, she moves freely between the orders, counseling patience and understanding. Her wisdom and compassion make her a bridge between Cassandra's zealotry and Vladimir's malice." The second character is placed in the middle of "Good" and "Middle" and is close to "The Sighted Saviors...", with the description "Miranda Clearwater, 29, is a driven warrior-priestess in the Sighted Saviors. She has tirelessly honed her combat skills and tactical knowledge to become a supreme instrument of the order's campaign against magic. Though ruthless for her crusade, she retains some empathy and will ally with benign mystics against great evils." The third character is close to "Evil" and "The League of the Blind...", with the description of "Vladimir Skullreave, 67, is a ruthless psychic vampire and high priest of the League of the Blind who cares only for spreading suffering and death. His powerful visions and mind control abilities make him a dangerous foe to Eliza Caeles and the Sighted Saviors." b) Steering generation: In this part, the visual spaces between the concept "magnets" are used to steer the LLM generation. The user can specify weights for the considered concepts (indicated by a red circle) to influence the generation process. In the example, the red circle is placed in the middle between "Good implies..." and "Evil implies..." c) Correcting AI behaviors: This section illustrates how users can correct misalignments between LLM behaviors and their own perceptions. The user can either 1) revise the element's placement directly or 2) re-steer the generation by re-positioning the element. The corrections are then fed back into the LLM pipeline as examples for future steering and recognition tasks, which is noted with "Used to adjust AI behaviors."}
  \label{fig:teaser}
